A Deep Learning & Fast Wavelet Transform-based Hybrid Approach for Denoising of PPG Signals

This letter presents a novel hybrid method that leverages deep learning to exploit the multi-resolution analysis capability of the wavelets, in order to denoise a photoplethysmography (PPG) signal. Under the proposed method, a noisy PPG sequence of length N is first decomposed into L detailed coefficients using the fast wavelet transform (FWT). Then, the clean PPG sequence is reconstructed as follows. A custom feedforward neural network (FFNN) provides the binary weights for each of the wavelet sub-signals outputted by the inverse-FWT block. This way, all those sub-signals which correspond to noise or artefacts are discarded during reconstruction. The FFNN is trained on the Beth Israel Deaconess Medical Center (BIDMC) dataset under the supervised learning framework, whereby we compute the mean squared-error (MSE) between the denoised sequence and the reference clean PPG signal, and compute the gradient of the MSE for the back-propagation. Numerical results show that the proposed method effectively denoises the corrupted PPG and video-PPG signal.

==> section2.tex <==
\section{System Model and Problem Formulation}
\label{SM}
%_________________%


%%_________________________________________________________________________________%%

\begin{figure} 
\centering
\includegraphics[width=3.4in]{Figures/SM.PNG}
\caption{System Model}
\centering
\label{fig:SM}
\end{figure}

We have designed multi-level fast wavelet decomposition with neural network to remove the noise from PPG signal. An input noisy  signal of length N with the window size of 8sec is given to wave decomposition block. In this the signal is decomposed into detail $cD_n$ and approximate coefficients $cA_n$. The approximate coefficient at each level helps obtain the next level of coefficients. 

The same noisy input is imported into neural network which generates the neurons with the same output size as of decomposition. Dot product of the coefficients obtained from wave decomposition and values of output neuron is computed to obtain the reconstructed signal as shown in  Figure \ref{fig:SM}. Network is trained to update the neurons which helps cancels the effect of those coefficient which introduces artifact in the signal. Sharp spikes and noise will be eliminated from output signal.





==> section3.tex <==

% The objective of rate maximization problem is to find the optimal time for energy, information transmission and optimal IRS phase matrix in energy transmission, and information transmission phases. Thus, the maximum rate is the solution of following optimization problem,



% \subsection{Case 1: Single Antenna without Interference}
% When there is no interference present and M=1, eq.\ref{Es} and eq.\ref{gama_d} reduce to

% \begin{equation}\label{Es_opt}
%     P_{s1} = \eta \frac{\tau}{1- \tau} [P_B || \Bar{h}^H_{BS}+  \Bar{g}_{RS}^H \theta_{ET} G_{BR} ||^2 ]
% \end{equation}
% \begin{equation}\label{gama_d_opt} 
%     \gamma_{D1} = \frac{P_{s1}|h_{SD}+\Bar{g}^H_{RD} \theta_{IT} \Bar{g}_{SR}|^2}{\sigma^2_n}
% \end{equation}
% This special case results into following the convex optimization problem.

% \begin{equation*}
% \begin{aligned}
% \textbf{P1}: 
% & \ \ \underset{\theta_{et},\theta_{it}, \tau }{\text{maximize}}
% & & C_1 \\
% &  \ \ \text{subject to}
% & & |\theta_{et}(i)|= 1, \; i = 1, \ldots, N \\
% & & & |\theta_{it}(i)|= 1, \; i = 1, \ldots, N \\
% & & & 0 < \tau \leq 1 \\
% \end{aligned}
% \end{equation*}

% Where $C_1 = (1-\tau)\log_2(1+\gamma_{D1})$  which, in this case, follows from eq. \ref{Es_opt} and \ref{gama_d_opt}. It is easy to show that the optimal solution of P1 is,
% \begin{equation*}
%     \hat{\theta}_{et} = 
% \end{equation*}

% \begin{equation*}
%     \hat{\theta}_{it} = 
% \end{equation*}

% \begin{equation*}
%     \hat{\tau} = 
% \end{equation*}
% Where $\hat{\theta}_{et}$, $\hat{\theta}_{it}$ and  $\hat{\tau}$ are the optimal solutions of P1.

% \subsection{Case 2: Multiple Antennas without Interference}
% In the absence of interference when $M \ge 2$ the following optimization problem is formulated,
% \begin{equation*}
% \begin{aligned}
% \textbf{P2}: 
% & \ \ \underset{\theta_{et},\theta_{it}, \tau }{\text{maximize}}
% & & C_2 \\
% &  \ \ \text{subject to}
% & & |\theta_{et}(i)|= 1, \; i = 1, \ldots, N \\
% & & & |\theta_{it}(i)|= 1, \; i = 1, \ldots, N \\
% & & & 0 < \tau \leq 1 \\
% \end{aligned}
% \end{equation*}
% Where $C_2 = (1-\tau)\log_2(1+\gamma_D)$  which, in this case, follows from eq. \ref{Es_opt} and \ref{gama_d_opt}. Although, P2 looks similar to P1 but it can be shown that P1 turn turns out to be non-convex problems as we increase M.Therefore, P2 is much difficult to solve due to its non-convex nature. 
% Here its worth mentioning that $G_{BR} \in \mathbb{C}^{M x N} $ rather than $\mathbb{C}^{1 x N}$ which makes P2 different from P1.






